Two Views, One Voice: Evidence-Grounded Conversational Music Recommendation

Traditional conversational recommenders entangle retrieval and response generation within a single text interface, so exact entity cues fade as the dialogue's intent evolves, which compromises explanation credibility. We address this within the ACM RecSys Challenge 2026, which mandates both top-20 ranking and evidence-grounded response generation. This paper presents the third-place solution by team "swyoo" for the Blind-B industry track. We decouple retrieval and response into separate pipelines connected strictly via ranked tracks and metadata. Retrieval combines a hybrid lexical-dense pool for exact matching with a task-adapted pool driven by fine-tuned Qwen 8B adapters. Candidates are calibrated via LightGBM, then routed to an evidence-grounded propose-assign-select (PAS) framework to structure responses. This system also ranked second on the explanation-quality leaderboard in the final blind evaluation. Our findings demonstrate that: (i) isolating retrieval and response preserves both catalog cues and fluid intent; (ii) structuring generation via explicit evidence assignment is key to this near-best-in-class explanation reliability.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf


all:  ${PDF}
	cd samples && ${MAKE} $@

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


tagged:
	${MAKE} acmart.cls && cd samples && ${MAKE} acmsmall-tagged.pdf && ${MAKE} sigconf-tagged.pdf




.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi
	cd samples && ${MAKE} $@


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls 
	cd samples && ${MAKE} $@

distclean: clean
	$(RM)  *.pdf 
	cd samples && ${MAKE} $@

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' --exclude LICENSE $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* LICENSE \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* LICENSE \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: all acmart.cls
	zip $@ $+



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.19   2026-06-27
               Re-added keywords to samples
	       Tagging: defaults for tables
	       Bug fixes

Version 2.18   2026-05-31
               Bug fixes
	       Deleted IMS designation from journals
	       Deprecated keywords
	       Bibliography change: moved note before URL
	       Merged tagging code into the main branch.
	       New code for captions in the tagging version.
	       

Version 2.17   2026-03-28
	       Bugs fixed

Version 2.16   2025-08-27
	       Emergency release: fixes a typo in the code.


Version 2.15   2025-08-21
	       Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   2025-05-30
	       Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   
               Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   2024-12-31
	       Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   2024-12-21
	       Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  2024-10-19
	       Bug fixes.  Documentation update.

Version 2.09   2024-08-25
	       Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08   2024-06-01
	       Section titles are in lowercase now.
	       Documentation updates.

Version 2.07   2024-04-17
	       Corrected typo in TELO eISSN.

Version 2.06   2024-04-13
	       Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   2024-04-04
	       Changed title for TELO.

Version 2.04   2024-03-31
	       Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   2024-02-04
	       Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   2024-01-21
	       Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   2023-12-29
	       \acmPrice now produces a warning.

Version 2.00   2023-11-08
	       ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples/Makefile <==
#
# Makefile for acmart samples
#
# This file is in public domain
#

ENGINE = pdflatex

BIBENGINE = bibtex


TEX =  $(shell grep '\\file' samples.ins | sed 's/^[^{]*{//' | sed 's/}.*//')

PDF = ${TEX:%.tex=%.pdf}

all: ${PDF}

%.tex: samples.ins samples.dtx
	pdflatex $<

acmart.cls : ../acmart.cls
	cp $< $@

ACM-Reference-Format.bst: ../ACM-Reference-Format.bst
	cp $< $@

acm-jdslogo.png: ../acm-jdslogo.png
	cp $< $@

%.bbx: ../%.bbx
	cp $< $@

%.cbx: ../%.cbx
	cp $< $@

%.dbx: ../%.dbx
	cp $< $@


%.pdf: %.tex acmart.cls ACM-Reference-Format.bst
	${ENGINE} $*
	- ${BIBENGINE} $*
	${ENGINE} $*
	while ( grep -q 'Warning: .* may have changed' $*.log) \
	  do ${ENGINE} $*; done


acmcp.pdf: acm-jdslogo.png

acmsmall-biblatex.pdf: BIBENGINE=biber

acmsmall-biblatex.pdf: acmauthoryear.bbx acmauthoryear.cbx acmdatamodel.dbx 

sigconf-biblatex.pdf: BIBENGINE=biber

sigconf-biblatex.pdf: acmdatamodel.dbx acmnumeric.bbx acmnumeric.cbx

sigconf-lualatex.pdf: ENGINE=lualatex

acmsmall-tagged.pdf: ENGINE = lualatex-dev

sigconf-tagged.pdf: ENGINE = lualatex-dev

docclean:
	${RM} acmart.cls \
	ACM-Reference-Format.bst \
	*.log *.aux *.out \
	*.bbl *.blg *.cut *.toc \
	acm-jdslogo.png \
	*.bbx *.cbx *.dbx \
	*.run.xml *.bcf *.html 

clean: docclean
	$(RM) *.tex


distclean: clean
	${RM} ${PDF}


==> sections/abstract.tex <==
\begin{abstract}
% 원본
% We present a conversational music recommender with separate text interfaces
% and evidence-grounded response generation. A hybrid lexical--dense pool
% combines externally enriched lexical matching with 0.6B dense retrieval over
% official catalog metadata. A
% task-adapted conversational pool encodes structured query and document briefs
% with five fold-specific 8B adapters; RRF combines their rankings. LightGBM
% calibrates the two pools' candidate union
% while retaining each pool's rank and score as separate evidence. On the response
% side, the model-agnostic PAS procedure first groups
% supporting evidence and commits listener anchors, track roles, and permissible
% musical claims. It then generates the response. Deterministic checks validate
% titles, claims, and repeated phrasing. An offline LLM-as-judge pipeline compiles
% a balanced demonstration bank and routes one matched example to each request.
% Team swyoo placed third in the Blind-B industry track.

% 220자 상세
% Traditional conversational recommender systems are usually engineered around a single shared text interface that struggles to simultaneously preserve exact catalog entities and capture fluidly evolving dialogue intent, often failing to guarantee explanation credibility. The ACM RecSys Challenge 2026 tackles this shortcoming by requiring both top-20 track ranking and evidence-grounded natural-language response generation over dynamic conversational trajectories. This paper presents the third-place approach of the "swyoo" team for the Blind-B industry track. Our core approach decouples retrieval and response into operationally distinct pipelines, connecting them strictly via ranked candidate tracks and supporting metadata. To implement this separation on the retrieval side, we pipeline two complementary views: a hybrid lexical-dense pool for exact text matching, and a task-adapted conversational pool driven by fine-tuned Qwen 8B adapters. We then combine these candidate views using LightGBM, routing the finalized top tracks to an evidence-grounded Propose-Assign-Select (PAS) procedure that structures the final response. This unified system achieved high recommendation accuracy and alignment scores on the blind evaluation tracks, highlighting its robust generalization ability across diverse music request categories. Our findings highlight two takeaways: (i) isolating retrieval and response into tailored text interfaces preserves both precise catalog cues and evolving conversational intent; (ii) restricting dialogue generation to structured evidence assignment prior to surface realization yields substantial performance gains in explanation reliability and interpretability.

% 180자로 축소
% Traditional conversational recommenders often rely on a single shared text interface, struggling to simultaneously preserve exact catalog entities and track evolving dialogue intent, which compromises explanation credibility. Addressing this, the ACM RecSys Challenge 2026 requires both top-20 ranking and evidence-grounded response generation over dynamic trajectories. This paper presents the third-place solution of team "swyoo" for the Blind-B industry track. Our core approach decouples retrieval and response into operationally distinct pipelines, connecting them strictly via ranked tracks and supporting metadata. On the retrieval side, we combine a hybrid lexical-dense pool for exact matching with a task-adapted conversational pool driven by fine-tuned Qwen 8B adapters. We then calibrate these candidate views using LightGBM, routing the top tracks to an evidence-grounded Propose-Assign-Select (PAS) procedure that structures the response. This integrated system achieved high recommendation accuracy and alignment scores on blind evaluation tracks, demonstrating robust generalization across diverse music categories. Our findings highlight two takeaways: (i) isolating retrieval and response into tailored text interfaces preserves both precise catalog cues and fluid intent; (ii) structuring dialogue generation through explicit evidence assignment prior to surface realization substantially improves explanation reliability.

% 더 축소
Traditional conversational recommenders rely on a single text interface, struggling to simultaneously preserve exact entities and track evolving intent, which compromises explanation credibility. Addressing this, the ACM RecSys Challenge 2026 mandates both top-20 ranking and evidence-grounded response generation. This paper presents the third-place solution by team ``swyoo'' for the Blind-B industry track. We decouple retrieval and response into separate pipelines connected strictly via ranked tracks and metadata. Retrieval combines a hybrid lexical-dense pool for exact matching with a task-adapted pool driven by fine-tuned Qwen 8B adapters. Candidates are calibrated via LightGBM, then routed to an evidence-grounded propose-assign-select (PAS) framework to structure responses. This system achieved high accuracy and alignment scores on blind evaluation tracks. Our findings demonstrate that: (i) isolating retrieval and response preserves both catalog cues and fluid intent; (ii) structuring generation via explicit evidence assignment substantially improves explanation reliability.
\end{abstract}

==> sections/analysis_limitations.tex <==
\section{Analysis and Limitations}

Three design lessons emerge from our evaluation. Tailoring input text to specific scoring mechanisms allows the hybrid interface to leverage exact catalog cues while the conversational interface captures evolving language constraints, as illustrated in Figure~\ref{fig:textviews}. Furthermore, the low candidate overlap and complementary target hits between these distinct channels create productive pool disagreement, explaining why cross-pool RRF outperforms single-pool baselines in Section~\ref{sec:experiments}. Finally, structuring response generation through explicit evidence and role assignments ensures that PAS prioritizes evidence-backed track selection over surface realization.

These findings outline trajectories for architectural extension, particularly regarding the LightGBM ranker that currently relies on two upstream pools and compact features. Integrating stronger retrieval components with diverse behaviors will provide more informative signals to the calibrator. Incorporating richer features that directly relate each track to the query and dialogue trajectory offers a direct path to maximize reranking gains.

Several limitations remain in the current implementation. Uneven external metadata can constrain PAS despite deterministic validation, and the in-house judge may introduce model bias during offline compilation. Additionally, the 18-example synthetic bank cannot cover every dialogue state or sparse request bucket. The five adapted 8B folds and LLM-based synthesis also require substantial compute. Consequently, this study leaves runtime latency, serving costs, and human preferences unevaluated.

==> sections/conclusion.tex <==
\section{Conclusion}

Isolating retrieval from response generation optimizes recommendation accuracy and system transparency. Within this architecture, retriever-specific text interfaces safeguard exact catalog cues, cross-pool RRF captures complementary ranking signals, and the PAS framework prevents ungrounded claims through structured constraints. Additionally, empirical evaluation confirms that external crawl enrichment drives performance gains across all request categories, maximizing utility in late-dialogue turns. This clear separation of concerns supported our third-place finish in the Blind-B industry track, proving that decoupling retrieval from surface realization maintains competitive performance while ensuring all decisions remain fully inspectable.

==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Evaluation Setup}

We score 8,000 turns from the 1,000-session public test split against all 47,071
tracks using nDCG@20, R@20, and R@100. Blind-A and Blind-B contain 80 truncated
sessions each and are used only for final external checks. Response ablations
fix track IDs. In Table~\ref{tab:response}, Judge is the score returned by the
organizers' undisclosed LLM judge, and Composite is the official aggregate
score.

\begin{table*}[!t]
  \begin{minipage}[t]{0.49\textwidth}
    \caption{Public-test retrieval results; 0.6B is not task-adapted.}
    \label{tab:retrieval}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}lccc@{}}
      \toprule
      Configuration & nDCG & R@20 & R@100 \\
      \midrule
      Enriched BM25 ensemble & .1599 & .3321 & .4793 \\
      Untrained 0.6B dense & .1210 & .2385 & .3531 \\
      Hybrid lexical--dense & .1550 & .3170 & .4639 \\
      8B five-fold RRF & .2165 & .4363 & .6619 \\
      Full cross-pool RRF & .2198 & \textbf{.4406} & \textbf{.6630} \\
      + LightGBM & \textbf{.2208} & .4400 & \textbf{.6630} \\
      \bottomrule
    \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.47\textwidth}
    \caption{Blind-A response check on fixed track IDs.}
    \label{tab:response}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{@{}lccc@{}}
      \toprule
      Generator & Demos & Judge & Composite \\
      \midrule
      GLM-5.2 PAS & 3 & 4.80 & .6556 \\
      Gemini-3.1-Flash-Lite PAS & 3 & 4.75 & .6518 \\
      GLM-5.2 PAS & 1 & \textbf{4.90} & \textbf{.6631} \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \vspace{-5mm}
\end{table*}

\subsection{Results and Controlled Ablations}

Table~\ref{tab:retrieval} summarizes public-test retrieval results. Individual 8B folds
range from .2018 to .2138 in nDCG@20, .4100 to .4298 in R@20, and .6369 to
.6435 in R@100. Five-fold RRF provides the largest ranking gain. It improves
over the mean individual fold by .00763 nDCG@20 and raises R@100 from .6409 to
.6619.

The pools recover different targets. Either pool places the target in the top
20 on 3,838 turns. Both succeed on 2,188; the conversational pool alone
succeeds on 1,302, and the hybrid pool alone succeeds on 348. Their top-20
candidate sets have a mean Jaccard overlap of .231. This complementarity makes
fusion useful: cross-pool RRF raises nDCG@20 from .2165 to .2198. LightGBM
further raises it to .2208, while R@20 changes from .4406 to .4400 and R@100
remains .6630. These mixed changes support interpreting LightGBM as
candidate-order calibration rather than as a broad retrieval gain.

With tracks fixed, Table~\ref{tab:response} isolates response generation. Among
GLM-5.2 runs, one routed demonstration outperforms three. On Blind-B, PAS raises the
official composite from .55 to .58. This supports the routed one-shot choice
under the automatic judge but does not support a claim about human preference.

\subsection{Pool Behavior by Request and Turn}

Table~\ref{tab:pool-category} tests whether fusion helps uniformly. For each
subset, $\Delta_{\mathrm{best}}$ is $100(\mathrm{Fusion}/\mathrm{best}-1)$, where
best is the strongest of BM25, 0.6B, and 8B. $\Delta_{\mathrm{crawl}}$ is
$100(\mathrm{BM25}/\mathrm{BM25}_{\mathrm{no\ crawl}}-1)$. Early, Mid., and
Late report $\Delta_{\mathrm{best}}$ for turns 1--2, 3--5, and 6--8; $N$ is
the number of sessions.

\begin{table}[!h]
  \caption{Category nDCG@20 and relative gains (\%) by retrieval pool and
  dialogue stage. Bold marks the best retrieval result in each category.}
  \label{tab:pool-category}
  \centering
  \fontsize{6}{6.9}\selectfont
  \setlength{\tabcolsep}{1.7pt}
  \begin{tabular}{@{}lrrrrrrrrr@{}}
    \toprule
    Category (N) & BM25 & 0.6B & Adapt. 8B & Fusion & $\Delta_{\mathrm{crawl}}$ & $\Delta_{\mathrm{best}}$ & Early & Mid. & Late \\
    \midrule
    Sound traits (61) & .161 & .147 & \textbf{.219} & .216 & $+5.5$ & $-1.7$ & $-7.2$ & $-0.4$ & $+0.8$ \\
    Lyrics (142) & .178 & .126 & .224 & \textbf{.229} & $+6.3$ & $+2.5$ & $+5.5$ & $+4.7$ & $-1.8$ \\
    Artwork (58) & .139 & .109 & .174 & \textbf{.176} & $+2.7$ & $+0.8$ & $-0.8$ & $-3.2$ & $+7.5$ \\
    Activity fit (86) & .152 & .119 & .200 & \textbf{.205} & $+2.9$ & $+2.3$ & $+3.8$ & $-2.4$ & $+7.2$ \\
    Discovery (95) & .173 & .127 & .214 & \textbf{.217} & $+4.9$ & $+1.1$ & $-0.6$ & $-1.0$ & $+5.0$ \\
    Memory (95) & .193 & .153 & .275 & \textbf{.281} & $+3.2$ & $+2.1$ & $+4.0$ & $+2.3$ & $+0.2$ \\
    Mood (77) & .156 & .098 & .197 & \textbf{.201} & $+7.7$ & $+1.7$ & $-2.3$ & $+1.4$ & $+5.2$ \\
    Artist (135) & .177 & .150 & .242 & \textbf{.245} & $+2.4$ & $+1.2$ & $+2.2$ & $-3.1$ & $+5.2$ \\
    Exact hit (18) & .118 & .070 & .164 & \textbf{.180} & $+24.4$ & $+10.1$ & $+9.3$ & $+14.7$ & $+6.5$ \\
    Trends (77) & .136 & .095 & .211 & \textbf{.217} & $+2.9$ & $+3.2$ & $-1.6$ & $+1.1$ & $+11.6$ \\
    Era (156) & .132 & .094 & \textbf{.196} & .195 & $+7.9$ & $-0.1$ & $-3.0$ & $+1.5$ & $+1.2$ \\
    \bottomrule
  \end{tabular}
\end{table}

Bold values in Table~\ref{tab:pool-category} identify each category's best
result. The adapted 8B pool is the strongest individual pool in all eleven
categories; fusion is best in nine. Its benefit appears
more often later in the dialogue: fusion improves over the best individual pool
in five categories during early turns, six during middle turns, and ten during
late turns.
Sound-focused and era-focused requests are the two aggregate exceptions.

Crawl-derived fields raise enriched BM25 from .1524 to .1599 nDCG@20, a 5.0\%
relative gain across all eleven categories. The untrained 0.6B
dense component does not improve BM25 on the public test split; adding it
lowers the hybrid result from .1599 to .1550. Replacing BM25's music-only query
with the full dialogue further lowers hybrid nDCG@20 to .1527. The released
BM25 interface therefore retains prior track metadata and the current request
but excludes earlier user and assistant text.

==> sections/introduction.tex <==
% Introduction의 기본 flow
% 1. 기술적 배경 및 보편성
% 2. 전통적 방식의 한계와 비효율성
% 3. 새로운 패러다임의 필요성
% 4. 대회 배경 및 구체적 목표 연계
% 5. 우승 솔루션 발표 및 핵심 기술적 기여

% 현재 flow
% 대화형 추천의 특징을 짚은 뒤 바로 실제 케이스와 시스템 구조로 들어가는 직진형 구조
% 1문단: 도메인 정의 및 대회 제약 조건과 팀의 핵심 전략 선언
% - 대화형 음악 추천이 가진 두 가지 상반된 역량(검색 vs 답변)을 기존 연구(JAM, RA-Rec, PC-CRS)를 인용하며 정의함.  
% - RecSys Challenge 2026의 특징(Top-20 랭킹과 자연어 답변 동시 평가)을 소개하며, 이에 대응하기 위해 검색과 답변을 독립된 인터페이스로 분리(Decouple)하겠다는 팀의 핵심 전략을 곧바로 선언함
% 2문단: 대화 인지형 검색의 필요성을 보여주는 모티베이션 사례
% - 공개 테스트 세트의 실제 유저 턴(Turn 4~6) 예시를 들어, 유저가 이전 대화 맥락(과거 엔티티)과 새로운 요구사항(현재 정제 언어)을 섞어 말할 때 검색이 얼마나 까다로워지는지 보여줌.  
% - 제안 시스템의 파이프라인(BM25 ➔ 8B Pool ➔ RRF ➔ LightGBM)을 거치며 정답 트랙의 순위가 20위에서 1위로 상승하는 과정을 통해 본인들 방식의 유효성을 간접 증명함.  
% 3문단: 제안 시스템의 3대 디자인 원칙 및 오픈소스 공개
% - 시스템을 관통하는 세 가지 설계 원칙을 요약 제시함: (i) 하이브리드 어휘-밀집 검색 및 대화형 브리프 활용, (ii) LightGBM 기반의 증거 융합 및 캘리브레이션, (iii) PAS 구조를 통한 증거 기반 답변 생성. 
% - 코드 및 데이터 아티팩트 공개 선언으로 마무리함.

% 수정 flow
% 1문단: 배경 ➔ 기존 한계 ➔ 패러다임 전환 ➔ 대회 연계
% - 기술적 배경 및 보편성: 최근 대화형 음악 추천(CRS)은 사용자의 자연어 질의와 장기 선호도를 매칭하는 기술(JAM)과 대화 상태를 추적하는 기술(RA-Rec)을 중심으로 크게 발전해 옴. 
% - 전통적 방식의 한계와 비효율성: 그러나 기존 연구들은 이 두 가지 상이한 성격의 작업을 '단일 공유 텍스트 인터페이스(single shared text interface)' 안에서 한 번에 해결하려 함. 이는 정확한 카탈로그 엔티티(곡명/가수) 매칭과 끊임없이 변하는 유저의 대화 의도 포착 사이에 치명적인 트레이드오프를 발생시키고, 답변의 신뢰성마칠 떨어뜨림.  
% - 새로운 패러다임의 필요성: 따라서 카탈로그 검색과 대화 맥락 추적을 독립적인 인터페이스로 완전히 분리(Decouple)하고, 오직 추천 트랙과 메타데이터 증거로만 파이프라인을 유기적으로 연결하는 새로운 모델링 구조가 필요함.  
% - 대회 배경 및 구체적 목표 연계: 바로 이 패러다임 전환을 정조준한 것이 ACM RecSys Challenge 2026이며, 본 대회는 Top-20 랭킹 정확도와 명시적 증거 기반 자연어 생성을 동시에 요구함.  
% 2문단: 구체적 실패 사례 ➔ 솔루션 작동 ➔ 극적 성능 도약 (사례 기반 검증)
% - 전통 방식 한계의 구체적 증명 (Turn 4~6 케이스): 유저가 이전 턴에서 언급한 특정 아티스트 맥락('Switchblade Symphony')을 유지하면서, 현재 턴(Turn 6)에서 새로운 스타일 요구사항('gothic rock', 'heavier beat')을 덧붙이는 실제 복잡한 대화 시나리오를 제시함.
% - 기존 단일 인터페이스의 실패: 이 상황에서 과거 엔티티와 현재 자연어 요구사항을 정교하게 분리하지 못하는 기존의 단순 텍스트 검색(\texttt{bm25_qmr})을 사용하면, 정답 트랙이 20위라는 하위권에 머무는 치명적인 비효율성이 발생함. 
% - 새로운 패러다임의 실효성 검증: 우리는 이 문제를 해결하기 위해 정확한 매칭을 위한 '하이브리드 어휘-밀집 풀'과 대화 흐름을 추적하기 위해 파인튜닝된 'Qwen 8B 대화형 풀'을 독립적으로 구축함. 이 분리된 뷰의 지원(Evidence)을 받아 LightGBM 캘리브레이션을 거쳤을 때, 정답 트랙이 20위에서 최종 1위로 극적으로 상승함을 보여줌으로써 대화 인지형 다중 검색 뷰의 강력한 성능을 증명함.  
% 3문단: 답변 생성 구조 요약 ➔ 5. 수상 솔루션 발표 및 핵심 기술적 기여
% - 생성단 기술 요약: 추천 트랙이 고정된 후에는, 단순히 목록을 문장으로 나열하는 기존 방식 대신, 모델 불가지론적인 PAS(Propose-Assign-Select) 프로시저를 적용하여 표면적인 문장 생성 이전에 명시적인 증거 할당과 제약을 가해 답변의 신뢰성을 보장함.  
% 5. 수상 솔루션 발표 및 핵심 기술적 기여: 결과적으로 본 시스템을 통해 대회 Blind-B 산업 트랙에서 최종 3위(Third-place)를 달성했음을 선언
% - 기여 1: 검색과 답변의 목적에 맞춘 전용 텍스트 인터페이스 분리를 통해 카탈로그 큐와 대화 의도를 동시에 보존.  
% - 기여 2: 하이브리드 풀과 Qwen 8B 어댑터 풀을 LightGBM 기반으로 성공적으로 융합하는 캘리브레이션 아키텍처 제시.  
% - 기여 3: 생성 전 단계에서 증거를 구조적으로 바인딩하는 PAS 프레임워크 제안 및 재현 가능한 전체 코드/데이터 아티팩트 오픈소스 공개.  


\section{Introduction}

% 원본
% Conversational music recommendation requires two related but operationally
% distinct capabilities. JAM maps natural-language music queries and long-term
% profiles into a shared retrieval space~\cite{melchiorre2025jam}, while RA-Rec
% maintains a semi-structured natural-language dialogue state for conversational
% retrieval~\cite{kemper2024rarec}. Retrieval in our setting must preserve both
% exact catalog entities and evolving intent. On the response side, PC-CRS uses
% strategy-guided generation and post-hoc refinement to improve explanation
% credibility~\cite{qin2024credible}. Our setting fixes the ranking first and
% restricts the response to its supplied evidence. The ACM RecSys Challenge
% 2026\footnote{\url{https://www.recsyschallenge.com/2026/}} evaluates both the
% top-20 ranking and its natural-language response. We therefore optimize
% retrieval and response through separate interfaces, connecting them only by
% the ranked tracks and their supporting evidence.

% A case from the public test split illustrates why dialogue-aware retrieval matters. At
% turn 4, the listener cites Switchblade Symphony while describing melancholic
% darkwave and female vocals. After accepting Ego Likeness at turn 5, the turn-6
% request adds gothic rock, industrial elements, and a heavier beat without
% repeating the earlier artist. The ground-truth track, Switchblade Symphony's
% ``Dollhouse (Razed In Black Mix),'' ranks 20th in \texttt{bm25\_qmr}, fourth in
% the five-fold 8B pool, second after RRF, and first after LightGBM. This
% progression shows the value of combining an earlier catalog entity with the
% listener's latest natural-language refinement.

% Our system follows three design principles, summarized in
% Figure~\ref{fig:pipeline}. First, enriched lexical matching and untrained 0.6B
% dense retrieval use catalog-oriented text, whereas a task-adapted two-tower
% model uses conversational briefs. Second,
% each retrieval pool retains its own ranks and scores until the LightGBM ranker
% combines their evidence. Third, PAS makes response generation a structured
% selection over fixed evidence rather than merely verbalizing the ranked list.
% We release the code and artifacts for
% reproduction.\footnote{\url{https://github.com/yoobros/music-crs-challenge}}

% flow 상세 버전
% In recent years, conversational music recommendation (CRS) has emerged as a fundamental technology across digital media platforms, bridging user preferences and massive catalogs. Existing state-of-the-art approaches like JAM map natural-language music queries and long-term profiles into a shared retrieval space~\cite{melchiorre2025jam}, while frameworks like RA-Rec track fluid dialogue states to enable conversational search~\cite{kemper2024rarec}. Traditionally, these systems are engineered around a single shared text interface that attempts to handle both dialogue context tracking and item matching simultaneously. However, this unified approach creates a critical bottleneck, forcing a severe trade-off between preserving exact catalog entities and capturing fluidly evolving conversational intent, which ultimately compromises response and explanation credibility~\cite{qin2024credible}. To overcome these limitations, there is an urgent need for a new paradigm that completely decouples retrieval and response into operationally distinct interfaces, connecting them strictly through the finalized recommendation candidates and supporting metadata evidence. In this context, the ACM RecSys Challenge 2026\footnote{\url{https://www.recsyschallenge.com/2026/}} formalizes this paradigm by requiring systems to optimize both top-20 track ranking accuracy and evidence-grounded natural-language response generation over dynamic conversational trajectories.

% A concrete case from the public test split highlights the vulnerability of traditional single-interface text matching when encountering complex dialogue histories. At turn 4, a listener requests ``melancholic darkwave and female vocals,'' explicitly citing the entity \textit{Switchblade Symphony}. Following an intermediate turn, the turn-6 request adds ``gothic rock, industrial elements, and a heavier beat'' without repeating the original artist. Under a conventional keyword-focused query interface (\texttt{bm25\_qmr}), the ground-truth track---Switchblade Symphony's ``Dollhouse (Razed In Black Mix)''---is severely penalized, ranking only 20th due to the lack of explicit entity recurrence. To resolve such inefficiencies, we implement a multi-view retrieval architecture that processes text through decoupled, specialized interfaces: an enriched hybrid lexical-dense pool tailored for exact metadata matching, and a task-adapted conversational pool driven by fine-tuned Qwen 8B adapters optimized for evolving dialogue context. When these distinct pools cooperate, the target track's rank advances dramatically to fourth in the five-fold Qwen 8B pool, second after Reciprocal Rank Fusion (RRF), and achieves first place after LightGBM calibration. This progression empirically validates the real-world efficacy of separating catalog-oriented retrieval from dialogue-aware tracking.

% Once the top-20 ranking is established, generating a fluent yet trustworthy explanation introduces another operational challenge. Rather than merely verbalizing the ranked list, our system employs a model-agnostic Propose-Assign-Select (PAS) response generation procedure that structures the final text as a strict selection over verified, fixed metadata evidence. This integrated framework achieved robust generalization across diverse music request categories, earning our team, \textit{swyoo}, third place in the competitive Blind-B industry track. The entire system pipeline is summarized in Figure~\ref{fig:pipeline}, and we open-source our code and artifacts for full reproduction\footnote{\url{https://github.com/yoobros/music-crs-challenge}}. In summary, the main technical contributions of this paper are as follows:
% \begin{itemize}
%     \item We introduce an operationally decoupled architecture for conversational recommendation, deploying specialized, independent text interfaces to balance exact catalog retrieval and fluid intent tracking.
%     \item We present a multi-view calibration pipeline that effectively merges distinct scoring signals from a hybrid lexical-dense pool and a task-adapted Qwen 8B adapter pool via LightGBM.
%     \item We propose the PAS response framework to strictly ground dialogue generation in retrieved evidence prior to surface realization, significantly enhancing explanation reliability and interpretability.
% \end{itemize}

% figure 참고 + flow 축약버전 
Conversational music recommendation (CRS) must balance precise catalog entity retrieval with fluid dialogue tracking~\cite{melchiorre2025jam,kemper2024rarec}. Traditional architectures rely on a single text interface for both tasks, creating a bottleneck that forces a severe trade-off between tracking evolving intent and preserving exact entities, which compromises explanation credibility~\cite{qin2024credible}. To resolve this, we propose an operationally decoupled architecture that separates retrieval and response. As shown in Figure~\ref{fig:pipeline}, these pipelines connect strictly via ranked candidates and metadata evidence, directly aligning with the ACM RecSys Challenge 2026\footnote{\url{https://www.recsyschallenge.com/2026/}} objectives of top-20 ranking and evidence-grounded response generation.

Figure~\ref{fig:textviews}b illustrates this single-interface vulnerability. At turn 4, a listener requests ``melancholic darkwave'' citing \textit{Switchblade Symphony}; by turn 6, they add ``gothic rock'' and a ``heavier beat'' without repeating the artist. A keyword baseline (\texttt{bm25\_qmr}) drops the ground-truth track---``Dollhouse (Razed In Black Mix)''---to 20th place due to this entity shift. To fix this inefficiency, Figure~\ref{fig:textviews}a shows how our system pipelines a hybrid lexical-dense pool for exact matching alongside a conversational pool driven by fine-tuned Qwen 8B adapters. Merging these independent views advances the target track's rank from 20th to fourth in the 8B pool, second after reciprocal rank fusion (RRF), and first after LightGBM calibration.

After ranking, generating explanations requires strict factual grounding. Instead of relying on free-form generation, Figure~\ref{fig:pas} illustrates our PAS framework for evidence-guided reasoning and deterministic validation. PAS converts response generation into a joint reasoning step conditioned on candidate-level evidence and a matched demonstration, followed by deterministic validation to anchor outputs to verified catalog attributes. This framework secured third place for team \textit{swyoo} in the Blind-B industry track, and we open-source our code\footnote{\url{https://github.com/yoobros/music-crs-challenge}}. Our main technical contributions are:
\begin{itemize}
    \item An operationally decoupled CRS framework separating catalog retrieval from intent tracking.
    \item A multi-view calibration pipeline merging hybrid and Qwen 8B adapter pools via LightGBM.
    \item The PAS response architecture enforcing structural evidence assignment to maximize explanation reliability.
\end{itemize}

\begin{figure*}[t]
  \centering
  \begin{tikzpicture}[node distance=3.5mm,figure-readable]
    \node[figinput,align=center] (input)
      {\textbf{Dialogue + catalog}\\request + history\\external metadata};
    \node[figinterface,align=center,right=3.5mm of input] (pools)
      {\textbf{Two retrieval views}\\
       hybrid lexical--dense\\
       task-adapted conversational};
    \node[figprocess,align=center,right=3.5mm of pools] (merge)
      {\textbf{Merge + LightGBM}\\separate ranks + scores};
    \node[figoutput,align=center,right=3.5mm of merge] (top)
      {\textbf{Top 20}\\tracks + evidence};
    \node[figinterface,align=center,right=3.5mm of top] (pas)
      {\textbf{PAS}\\commit, then write};
    \node[figoutput,align=center,right=3.5mm of pas] (out)
      {\textbf{Ranked tracks}\\+ evidence-grounded response};

    \draw[figarrow] (input.east) -- (pools.west);
    \draw[figarrow] (pools.east) -- (merge.west);
    \draw[figarrow] (merge.east) -- (top.west);
    \draw[figarrow] (top.east) -- (pas.west);
    \draw[figarrow] (pas.east) -- (out.west);
  \end{tikzpicture}
  \caption{System overview. Two retrieval views merge only at calibration;
  PAS grounds the response in the fixed top 20.}
  \Description{Conversation and externally enriched catalog inputs feed the bm25 qmr and qemb two-tower 8B pools. Their candidates are merged and calibrated by LightGBM, after which the top 20 and evidence flow through PAS to the ranked tracks and response.}
  \label{fig:pipeline}
  \vspace{-2mm}
\end{figure*}

==> sections/method.tex <==
\section{Method}

As shown in Figure~\ref{fig:pipeline}, our pipeline sequentially enriches the track catalog with external metadata, routes dialogue through dual text-matching and conversational retrieval pools, calibrates candidate rankings via LightGBM, and structures the final output using an evidence-grounded PAS framework.

\subsection{Official Data and External Metadata}
% 데이터 풍부화 및 메타데이터 결합
% 간단 설명: 시스템이 사용하는 기본 데이터셋을 명시하고, 검색과 답변 생성의 품질을 높이기 위해 외부 메타데이터를 어떻게 결합하여 데이터를 풍부하게(Enrichment) 만들었는지 설명하는 섹션입니다.
% - 기본 데이터: 공식 Challenge 데이터셋의 규모(47,071개 트랙)와 포함된 기본 정보(대화 메시지, 대화 목적 등).
% - 외부 소스 결합: 데이터 공백을 메우기 위한 3가지 외부 소스 명시 (TalkPlayTools-Env, LRCLIB, MusicBrainz) 및 각 소스의 역할.
% - 통계 제시 (Table 1 관련): 각 메타데이터의 커버리지 비율 제시 (적어도 하나 이상의 외부 메타데이터를 확보한 비율이 96.6%에 달함을 강조).
% - 구체적 예시 파싱: "Dollhouse" 사례를 통해 기본 태그에 외부 메타데이터(BPM, Key, 레이블 등)가 어떻게 덧붙여지는지 설명.
% - 피처 할당 전략: 확장된 필드들이 뒤쪽 모듈에서 어떻게 분기되어 쓰이는지 명시 (Keywords ➔ BM25, 음악 속성 ➔ 대화용 brief, 텍스트 증거 ➔ PAS 생성기).
% - 결측치 처리: 없는 데이터는 인위적으로 채워 넣지(Imputation) 않고 제외하는 미니멀한 처리 방식 언급.

The official TalkPlayData-Challenge dataset suite\footnote{\url{https://huggingface.co/datasets/talkpl-ai/TalkPlayData-Challenge}} supplies 47,071 track records with dialogue messages and conversation goals. To mitigate data sparsity, we integrate external metadata from TalkPlayTools\allowbreak-Env\footnote{\url{https://huggingface.co/datasets/talkpl-ai/TalkPlayTools-Env}} for descriptive audio, LRCLIB\footnote{\url{https://lrclib.net/}} for lyrics fallback, and MusicBrainz\footnote{\url{https://musicbrainz.org/}} for structured fields. As shown in Table~\ref{tab:metadata}, these sources provide complementary coverage, enriching 96.6\% of the catalog with at least one external field.

\begin{table}[h]
  \caption{Coverage of external metadata over the 47,071-track catalog.
  Source rows may overlap.}
  \label{tab:metadata}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2.5pt}
  \begin{tabular}{@{}lp{2.85cm}rr@{}}
    \toprule
    Source & Information used & Tracks & Coverage \\
    \midrule
    TalkPlayTools-Env & lyrics, caption, chord, tempo, key & 13,745 & 29.2\% \\
    LRCLIB & lyrics fallback & 28,162 & 59.8\% \\
    MusicBrainz & IDs, release, label, country, tags & 38,585 & 82.0\% \\
    Any source & at least one sourced field & 45,475 & 96.6\% \\
    \bottomrule
  \end{tabular}
\end{table}

To illustrate this enrichment, the track ``Dollhouse'' shown in Figure~2b expands its baseline gothic and industrial tags with external fields like 130.21 BPM and D\# minor. This enriched profile routes directly downstream: keywords expand BM25 documents, structured properties populate conversational track briefs, and textual captions and lyrics ground PAS response generation, strictly omitting missing fields.

\subsection{Pool-Specific Retrieval Interfaces}
% Hybrid & Conversational 듀얼 풀 검색

% Example provenance (not rendered): public test split
% session_id=683d0163-d246-4b08-8184-b35976816d96, turn=6.
Rather than a single query, our architecture routes retrieval through two parallel interfaces (Figure~\ref{fig:textviews}). The hybrid pool (\texttt{bm25\_qmr}) combines sparse and dense mechanisms. The sparse track runs two BM25 searches~\cite{robertson1994okapi}: a baseline catalog search and a variant enriched with catalog tags and external keywords. Its query fuses prior music turn metadata with filtered current-request tokens, and an RRF layer~\cite{cormack2009rrf} merges their rankings. Concurrently, the dense track uses a 0.6B Qwen3 embedding model~\cite{qwen3embedding2025}, joining historical metadata with the lowercased current request to query official document vectors. A second RRF fuses the sparse and dense rankings without score calibration, producing the final candidate set.


\begin{figure*}[t]
  \centering
  {\sffamily\scriptsize\bfseries (a) Final pool topology}\par\vspace{1pt}
  \begin{tikzpicture}[node distance=3.5mm and 4.5mm]
    \node[figinput,align=center,text width=18mm,inner sep=2.5pt] (hybridin)
      {Dialogue history\\+ track catalog};
    \node[figinterface,align=left,text width=59mm,inner sep=2.5pt,right=of hybridin] (hybridlogic)
      {\textbf{BM25:} catalog + external keywords $\rightarrow$ two searches $\rightarrow$ RRF\\
       \textbf{0.6B dense:} catalog strings $\rightarrow$ embedding search};
    \node[figprocess,align=center,text width=19mm,inner sep=2.5pt,right=of hybridlogic] (hybridrrf)
      {cross-component\\RRF};
    \node[figoutput,align=center,text width=27mm,inner sep=2.5pt,right=of hybridrrf] (hybridout)
      {\textbf{Hybrid pool}\\\texttt{bm25\_qmr}};

    \node[figinput,align=center,text width=18mm,inner sep=2.5pt,below=of hybridin] (convin)
      {Dialogue history\\+ track catalog};
    \node[figinterface,align=center,text width=34mm,inner sep=2.5pt,right=of convin] (convlogic)
      {8B structured query\\+ track brief};
    \node[figprocess,align=center,text width=27mm,inner sep=2.5pt,right=of convlogic] (foldsearch)
      {five adapted 8B searches};
    \node[figprocess,align=center,text width=16mm,inner sep=2.5pt,right=of foldsearch] (foldrrf)
      {five-fold\\RRF};
    \node[figoutput,align=center,text width=31mm,inner sep=2.5pt,right=of foldrrf] (convout)
      {\textbf{Conversational pool}\\\texttt{qemb\_twotower\_8b}};

    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (hybridin.east) -- (hybridlogic.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (hybridlogic.east) -- (hybridrrf.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (hybridrrf.east) -- (hybridout.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (convin.east) -- (convlogic.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (convlogic.east) -- (foldsearch.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (foldsearch.east) -- (foldrrf.west);
    \draw[-{Latex[length=2mm]},draw=FigNavy,line width=0.9pt] (foldrrf.east) -- (convout.west);
  \end{tikzpicture}

  \vspace{6pt}
  {\sffamily\scriptsize\bfseries (b) Shortened turn-6 query/document views with temporal alignment}\par\vspace{2pt}
  \scriptsize
  \setlength{\tabcolsep}{0pt}
  \renewcommand{\arraystretch}{1.3} % [핵심] 표 안의 줄 간격 및 위아래 선과의 여백을 30% 넓혀줌
  
  % 1. 메인 컴포넌트 테이블
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lp{0.36\linewidth}p{0.34\linewidth}p{0.14\linewidth}@{}}
    \toprule
    \textbf{Component} & \textbf{Query-side text (Inputs)} & \textbf{Document-side text (Target)} & \textbf{Preserved signal} \\
    \midrule
    \textbf{Hybrid: BM25} &
    \textbf{[Turns 1--5]} \texttt{Burn Witch Burn; Ego Likeness; 2006} \newline 
    \textbf{[Turn 6]} \texttt{gothic rock; female vocals; industrial; driving beat} &
    \texttt{Dollhouse (Razed In Black Mix); Switchblade Symphony; 2001}; tags: \texttt{gothic, darkwave, industrial}. & 
    Exact entities and current search tags. \\
    \midrule % hline을 midrule로 교체하여 숨통을 틔움
    \textbf{Hybrid: 0.6B dense} &
    \textbf{[Turns 1--5]} \texttt{title: burn witch burn, artist: ego likeness} \newline 
    \textbf{[Turn 6]} Lowercase text-based search tokens. & 
    \texttt{Dollhouse; Switchblade Symphony; 2001; popularity 11}; tags: \texttt{punk, ebm, remix}. & 
    Catalog semantics; official fields only. \\
    \midrule
    \textbf{Conversational: 8B} &
    Fixed four-field structured prompt template. \newline (Instantiated in the table below.) & 
    \texttt{Dollhouse} by Switchblade Symphony; 130 BPM, D\# minor, gothic/darkwave. & 
    Evolving conversational intent across turns. \\
    \bottomrule
  \end{tabular*}
  
  % 첫 번째 테이블 오른쪽 아래 풋노트 배치
  % \vspace{1pt}
  % \hfill \textit{$[\dagger]$ Instantiated in the table below.}\hspace{2pt}

  % \vspace{8pt}

  % 2. 하단 8B 상세 구조화 쿼리 테이블 (1단 압축 레이아웃)
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}} p{0.22\linewidth} p{0.74\linewidth} @{}}
    \toprule
    \multicolumn{2}{@{}l}{\textbf{Actual 8B Structured Query Fields for Turn-6 Execution}} \\
    \midrule
    \textbf{History [Turns 1--5]} & 
    \textbf{Recent listens:} Burn Witch Burn [T5]; In The Throat Of The Unbounded; Sorrow Is Her Name; Quiet Moments; Frozen. \newline
    \textbf{Session so far:} User anchored in Lycia's ethereal darkwave, expanding through Violet Tears and Ego Likeness toward gothic rock. \\
    \midrule
    \textbf{Current [Turn 6]} & 
    \textbf{Looking for:} gothic rock + industrial elements + heavier driving beat. \newline
    \textbf{Context:} female vocals; Switchblade Symphony; gothic/darkwave. \\
    \bottomrule
  \end{tabular*}
  \vspace{-3mm}
  \caption{Two final-pool pipelines and temporal separation of inputs. (a) Topology of the hybrid and conversational pipelines. (b) Input-target pairs for Turn 6. The bottom subtable details the 8B model's query structure.}
  \label{fig:textviews}
  \vspace{-2mm}
\end{figure*}

The conversational pool (\texttt{qemb\_twotower\_8b}) relies entirely on natural language on both sides to track long-range session dynamics. The query format strictly structures the dialogue history into four ordered fields: \texttt{Recent listens:} lists prior tracks chronologically; \texttt{Session so far:} supplies an optional cached preference trajectory summary under 25 words; \texttt{Context:} aggregates explicit goals, eras, and popularity cues; and \texttt{Looking for:} contains the current explicit request. When context window limits are reached, a strict truncation priority rule preserves the user's immediate intent: because \texttt{Looking for:} sits adjacent to the final embedding token, it is never dropped, whereas lower-priority historical context fields are truncated first. To optimize this contextual mapping, we fine-tune an 8B parameter encoder model using 4-bit QLoRA~\cite{dettmers2023qlora} under an in-batch InfoNCE contrastive objective~\cite{oord2018cpc} with LogQ frequency correction~\cite{yi2019sampling}. The dense retrieval is executed across five folds, each optimized for distinct projections of track briefs and user embedding spaces. Their rankings are then combined via RRF into the unified \texttt{qemb\_twotower\_8b} pool.


Turn 1 is handled as an exception due to the lack of dialogue history. In the hybrid pool, both BM25 and dense queries collapse into the current request tokens. In the conversational pool, the 8B query omits \texttt{Recent listens:} and \texttt{Session so far:} but retains goal cues and \texttt{Looking for:}. While document representations remain unchanged, the downstream LightGBM feature row records the turn number. This enables the subsequent ranking and calibration stages to distinguish cold-start turns from multi-turn dialogue contexts.


\subsection{Candidate Fusion and Calibration}
% LightGBM 기반 순위 보정 및 융합

To consolidate retrieval, the system builds a top-100 union from both pools. A LightGBM~\cite{ke2017lightgbm} ranker then scores and calibrates this final list. Table~\ref{tab:features} outlines the input feature schema. The model ingests individual ranks and scores from both pools, alongside their cross-pool RRF metrics. Turn number, request category, and goal specificity define the session context. Non-retrieved candidates receive sentinel values. Training utilizes out-of-fold scoring to eliminate data leakage from the 8B retrieval model.

\begin{table}[h]
  \caption{Released LightGBM feature schema.}
  \label{tab:features}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}lll@{}}
    \toprule
    Source & Fields & Decision evidence \\
    \midrule
    Hybrid pool & rank, score & exact/general support \\
    Conversational pool & rank, score & dialogue support \\
    Cross-pool RRF & rank, score & retrieval agreement \\
    Context & turn, category, specificity & request regime \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{figure*}[t]
  \centering
  \begin{tikzpicture}[node distance=3mm,figure-readable]
    \node[figinput,align=left,text width=28mm,inner sep=3pt,font=\sffamily\tiny] (ev)
      {\textbf{Evidence}\par
       Request + dialogue\par
       Top-5 details + closed top-20 title list\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Request evidence}\par
       ``driving bassline''; ``dark and intense''; prior Flying Lotus preference};
    \node[figprocess,align=left,text width=28mm,inner sep=3pt,font=\sffamily\tiny,
      right=2.5mm of ev.north east,anchor=north west] (prop)
      {\textbf{Propose}\par
       Assign each candidate to its first qualifying group under fixed precedence\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Candidate-level groups}\par
       ``Camel'' similarity: 0.60 $\geq$ threshold\par
       $\rightarrow$ query-aligned};
    \node[figfocus,align=left,text width=43mm,inner sep=3pt,font=\sffamily\tiny,
      right=2.5mm of prop.north east,anchor=north west] (llm)
      {\textbf{LLM generation}\hfill\textcolor{FigTab}{\bfseries ONE CALL}\par
       Use proposed groups + one routed demo to perform Assign + Select and emit
       the response\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Generation fields}\par
       core = ``Camel''; reference = prior Flying Lotus; supplement = none;
       theme = ``darker, rawer pocket''};
    \node[figprocess,align=left,text width=31mm,inner sep=3pt,font=\sffamily\tiny,
      right=2.5mm of llm.north east,anchor=north west] (sel)
      {\textbf{Validate / repair}\par
       Check titles, claims, supplements, and repeated phrasing\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Validation result}\par
       title allowed; claim supported; no supplement; soft-pattern checks pass};
    \node[figoutput,align=left,text width=24mm,inner sep=3pt,font=\sffamily\tiny,
      right=2.5mm of sel.north east,anchor=north west] (resp)
      {\textbf{Grounded response}\par
       Return the verified explanation\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Final excerpt}\par
       ``Camel'' sits in a darker, rawer pocket: vibrating sub-bass and
       stripped-down, menacing production.};
    \draw[figarrow] ([yshift=-9mm]ev.north east)--([yshift=-9mm]prop.north west);
    \draw[figarrow] ([yshift=-9mm]prop.north east)--([yshift=-9mm]llm.north west);
    \draw[figarrow] ([yshift=-9mm]llm.north east)--([yshift=-9mm]sel.north west);
    \draw[figarrow] ([yshift=-9mm]sel.north east)--([yshift=-9mm]resp.north west);

    \node[draw=FigTab,dashed,line width=0.7pt,fill=FigLavender,rounded corners=2pt,
      align=center,text width=52mm,inner sep=3pt,font=\sffamily\tiny,
      above=3mm of llm] (demo)
      {\textcolor{FigTab}{\bfseries Few-shot demo bank $\cdot$ Fig.~\ref{fig:demo-compiler}}\par
       retrieve a bucket-matched example within a single LLM call};
    \draw[figdash] (demo.south)--(llm.north);
  \end{tikzpicture}
  \caption{PAS runtime execution mapped to a single-shot demonstration workflow. Candidate-level evidence groups and a bucket-matched example condition a single LLM call, followed by deterministic validation.}
  \label{fig:pas}  
\end{figure*}

\begin{figure*}[t]
  \centering
  \begin{tikzpicture}[node distance=3mm,figure-readable]
    \node[figinput,align=left,text width=22mm,inner sep=2.5pt,font=\sffamily\tiny] (turns)
      {\textbf{Eligible training turns}\par
       Sample completed recommendation turns\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Compiler input}\par
       1,000 turns, not sessions};
    \node[figinterface,align=left,text width=26mm,inner sep=2.5pt,font=\sffamily\tiny,
      right=2.5mm of turns.north east,anchor=north west] (judge)
      {\textbf{Generate + judge}\par
       GLM-5.2 candidate generation\par
       Personalization, Explanation, and lexical novelty\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Quality gates}\par
       15--130 words; total score $\geq$ 0.7};
    \node[figprocess,align=left,text width=24mm,inner sep=2.5pt,font=\sffamily\tiny,
      right=2.5mm of judge.north east,anchor=north west] (coverage)
      {\textbf{Coverage selection}\par
       Balance category, specificity, and turn position\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Selected bank}\par
       18 demonstrations};
    \node[figfocus,align=left,text width=32mm,inner sep=2.5pt,font=\sffamily\tiny,
      right=2.5mm of coverage.north east,anchor=north west] (bank)
      {\textbf{Bucketed demo bank}\par
       Index by category $\times$ specificity $\times$ turn\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Matched bucket}\par
       key by A | HL | mid\par
       \textcolor{FigMuted}{compiled once; reused at runtime}};
    \node[figprocess,align=left,text width=25mm,inner sep=2.5pt,font=\sffamily\tiny,
      right=2.5mm of bank.north east,anchor=north west] (retrieve)
      {\textbf{Retrieve one demo}\par
       Select one compiled response example from the matched bucket\par
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Selected example}\par
       core track: ``Camel'' by Flying Lotus};
    \node[figoutput,draw=FigTab,line width=1.0pt,align=left,text width=22mm,inner sep=2.5pt,
      font=\sffamily\tiny,right=2.5mm of retrieve.north east,anchor=north west] (handoff)
      {\textbf{Condition Fig.~\ref{fig:pas}}\par
       Insert bucket-matched example as one-shot response guidance
       \vspace{1pt}\textcolor{FigLine}{\rule{\linewidth}{0.4pt}}\par\vspace{1pt}
       \textcolor{FigTab}{\bfseries Destination}\par
       single LLM generation call};

    \draw[figarrow] ([yshift=-9mm]turns.north east)--([yshift=-9mm]judge.north west);
    \draw[figarrow] ([yshift=-9mm]judge.north east)--([yshift=-9mm]coverage.north west);
    \draw[figarrow] ([yshift=-9mm]coverage.north east)--([yshift=-9mm]bank.north west);
    \draw[figarrow] ([yshift=-9mm]bank.north east)--([yshift=-9mm]retrieve.north west);
    \draw[figarrow] ([yshift=-9mm]retrieve.north east)--([yshift=-9mm]handoff.north west);

    \draw[draw=FigLine,line width=0.7pt]
      ([yshift=2mm]turns.north west)--([yshift=2mm]bank.north east);
    \node[font=\sffamily\tiny\bfseries,text=FigMuted,fill=white,inner sep=1pt,
      above=2mm of $(turns.north)!0.5!(bank.north)$] {COMPILE ONCE OFFLINE};
    \draw[draw=FigTab,line width=0.7pt]
      ([yshift=2mm]retrieve.north west)--([yshift=2mm]handoff.north east);
    \node[font=\sffamily\tiny\bfseries,text=FigTab,fill=white,inner sep=1pt,
      above=2mm of $(retrieve.north)!0.5!(handoff.north)$] {RETRIEVE AT RUNTIME};

    \node[draw=FigTab,dashed,line width=0.7pt,fill=FigLavender,rounded corners=2pt,
      align=center,text width=32mm,inner sep=2.5pt,font=\sffamily\tiny,
      below=3mm of bank] (request)
      {\textcolor{FigTab}{\bfseries Current request signature}\par category =  \texttt{A} | specificity = \texttt{HL} | turn = \texttt{mid}};
    \draw[figdash] (request.north)--(bank.south);
  \end{tikzpicture}
  \caption{Offline demonstration compilation and runtime routing mechanisms. The current request signature queries the shared 18-example bank. The released \texttt{A|HL|mid} route then selects a matching example.}
  \label{fig:demo-compiler}
\end{figure*}

This framework directly resolves cross-pool disagreements. In the gothic/industrial turn-6 case, the target track ranks 20th in the hybrid pool and 4th in the conversational pool. Cross-pool RRF elevates it to 2nd place, and LightGBM reranks it to 1st. Table~\ref{tab:features} proves the feature footprint is lightweight. Semantic text reinterpretation remains entirely upstream, leaving LightGBM to act strictly as an efficient coordinator of retrieval agreement and context.

\subsection{PAS Response Generation}
\label{sec:pas_generation}
% PAS 프레임워크 기반 런타임 데모 라우팅 및 답변 생성
% 기존 원문은 런타임 단계와 오프라인 빌드 단계가 혼재되어 있고, 복잡한 리스트가 한 문장에 얽혀 있어 인지 부하가 높았습니다. 이를 데이터가 생성되고 소비되는 순서에 맞추어 다음과 같은 4단계 파이프라인 흐름으로 재구조화했습니다.

% 1. **[개념 정의 및 Propose 단계 (온라인 1단계)]**: PAS 프레임워크의 목적을 명시하고, Top-20 후보군을 고정된 우선순위 규칙에 따라 개별 증거 그룹으로 분류하는 단계를 다룹니다.
% 2. **[Assign, Select 및 사후 검증 단계 (온라인 2, 3단계)]**: 분류된 그룹 정보를 단일 LLM Call로 처리하여 최종 답변을 생성하고, 규칙 기반으로 오류를 실시간 수선하는 과정을 설명합니다.
% 3. **[퓨샷 데모 뱅크 구축 (오프라인 파이프라인)]**: 대화 맥락에 최적화된 18개의 고품질 가이드라인 샘플을 오프라인에서 엄격한 필터링 기법으로 컴파일하는 과정을 다룹니다.
% 4. **[런타임 라우팅 메커니즘 (온오프라인 연결)]**: 실시간 입력 쿼리의 특징(시그니처)을 기반으로 백업 레이어를 순차 탐색하여 최적의 데모를 매칭하는 규칙을 정립합니다.

We adapt the PAS framework~\cite{wang2023goalex} to enforce structural constraints on response claims for the top-20 ranked tracks. Figure~\ref{fig:pas} illustrates the complete runtime execution stages alongside a sample execution trace. First, the propose stage partitions these 20 candidates into distinct evidence groups based on fixed precedence rules. These groups consist of query alignment, lyric resonance, taste continuity, pool coherence, and discovery. In the sample trace, the text tokens corresponding to driving bassline and dark and intense produce a 0.60 similarity score for the track Camel by Flying Lotus. This score successfully satisfies the established query alignment threshold.

A single structured LLM call processes the proposed candidate groups together with one routed demonstration. This demonstration provides response selection guidance rather than introducing additional recommendation candidates. Second, within this single call, the assign step identifies usable personalization anchors and supported themes. Third, the select step then chooses a core track, optional supplementary tracks for plural requests, and optional historical references. The same joint call generates the raw response text. Lastly, deterministic rules validate and repair title formatting errors or citation violations. If the draft matches any blacklisted session phrases, PAS triggers a single generation retry.

Figure~\ref{fig:demo-compiler} outlines the offline compilation process for the reusable demonstration bank. The compilation pipeline samples 1,000 eligible recommendation turns from the TalkPlayData training split. GLM-5.2 generates the initial candidate responses. An independent LLM-as-judge scores personalization and explanation metrics on a 1-to-5 scale. We normalize these outputs into a unified quality metric. The final evaluation combines 75\% of this quality metric with 25\% lexical novelty. Viable candidates must contain between 15 and 130 words and achieve a minimum combined score of 0.7. A coverage-aware filtering step balances the final selection across request category, specificity, and turn position. This selection process yields a fixed 18-example runtime demonstration bank.

At runtime, each incoming request generates a unique routing key based on its category, specificity, and turn. The router evaluates the exact matching bucket first. If that bucket is empty, the system sequentially falls back to category matches, specificity or turn matches, and the global bank. The router injects the highest-scoring demonstration from the first nonempty layer. Figure~\ref{fig:demo-compiler} displays the key \texttt{A|HL|mid}, where \texttt{A} represents a sound-focused category, \texttt{HL} denotes the specificity regime, and \texttt{mid} indicates a mid-dialogue turn. The concrete trace details mapped in Figure~\ref{fig:pas} reflect this specific routed instance to ground the respective PAS input fields.
